Do Neural Language Representations Learn Physical Commonsense?

Humans understand language based on the rich background knowledge about how the physical world works, which in turn allows us to reason about the physical world through language. In addition to the properties of objects (e.g., boats require fuel) and their affordances, i.e., the actions that are applicable to them (e.g., boats can be driven), we can also reason about if-then inferences between what properties of objects imply the kind of actions that are applicable to them (e.g., that if we can drive something then it likely requires fuel). In this paper, we investigate the extent to which state-of-the-art neural language representations, trained on a vast amount of natural language text, demonstrate physical commonsense reasoning. While recent advancements of neural language models have demonstrated strong performance on various types of natural language inference tasks, our study based on a dataset of over 200k newly collected annotations suggests that neural language representations still only learn associations that are explicitly written down.

==> src/related-work.tex <==
\section{Related Work}
\label{sec:relwork}

We are not the first to investigate affordances using techniques from machine learning. Recent insightful work by by \citeA{fulda2017can} extracted a global \textit{affordance vector} in word embedding space by averaging the a small set of chosen canonical pairs such as \textit{(read, book)} and \textit{(drink, water)}.

In visual reasoning problems, understanding what people might do to different objects in an image or video is beneficial in understanding a scene's composition and functionality. \citeA{fathi2011understanding} use images from an egocentric camera to construct representations of everyday activities. Several works employing affordances in visual domains have strong ties to robotics, using visual features to aid in object class detection or manipulation \cite{metta2003early,fritz2006learning,stark2008functional}. \citeA{koppula2016anticipating} use affordances to anticipate a person's goals and future trajectories, which has strong ties to work in visual activity recognition \cite{wu2007scalable,sung2012unstructured,donahue2015long}.

A rich line of work in NLP has studied the fundamental link between verbs and object properties in the context of frame semantics \citeA{fillmore1976frame,baker1998berkeley,kipper2000class,palmer2005proposition} as well as thematic and semantic proto-roles \cite{dowty1991thematic,reisinger2015semantic,zhang2016ordinal}.

\citeA{herbelot2015concepts} define a binned annotation layer (\textsc{all / most / some / few / none}) on top of the \citeA{mcrae2005semantic} data, though they keep the base set of elicitations and objects.
